AC-Teach: A Bayesian Actor-Critic Method for Policy Learning with an Ensemble of Suboptimal Teachers

The exploration mechanism used by a Deep Reinforcement Learning (RL) agent plays a key role in determining its sample efficiency. Thus, improving over random exploration is crucial to solve long-horizon tasks with sparse rewards. We propose to leverage an ensemble of partial solutions as teachers that guide the agent's exploration with action suggestions throughout training. While the setup of learning with teachers has been previously studied, our proposed approach - Actor-Critic with Teacher Ensembles (AC-Teach) - is the first to work with an ensemble of suboptimal teachers that may solve only part of the problem or contradict other each other, forming a unified algorithmic solution that is compatible with a broad range of teacher ensembles. AC-Teach leverages a probabilistic representation of the expected outcome of the teachers' and student's actions to direct exploration, reduce dithering, and adapt to the dynamically changing quality of the learner. We evaluate a variant of AC-Teach that guides the learning of a Bayesian DDPG agent on three tasks - path following, robotic pick and place, and robotic cube sweeping using a hook - and show that it improves largely on sampling efficiency over a set of baselines, both for our target scenario of unconstrained suboptimal teachers and for easier setups with optimal or single teachers. Additional results and videos at https://sites.google.com/view/acteach/home.

==> 0-preamble.tex <==
% Author: Animesh Garg
% Date : July 2015
% This is a list of common packages needed in a wide range of latex docs for everyday writing.
% ---------------------------------
%floats and figures
% ---------------------------------
\usepackage{graphics}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage[pdftex]{graphicx}
% \usepackage{wrapfig}
\DeclareGraphicsExtensions{.pdf,.png,.jpg}
%\pdfimageresolution200

\usepackage[skip=2pt,font=small]{caption}
\usepackage{subcaption}
%DONT USE BOTH SUBCAPTION AND SUBFIGURE
% \usepackage[center]{subfigure} 
% \usepackage{overpic}
\usepackage[rightcaption]{sidecap}
\usepackage{pbox}

% ---------------------------------
%Math Stuff
% ---------------------------------
\usepackage{mathtools}
\usepackage{amsmath, amssymb, amscd}
\usepackage{ wasysym } %special symbols
\usepackage{amsfonts}
\usepackage{mathptmx} % selects Times Roman as basic font
\usepackage{gensymb} 
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{mdwmath}
% \usepackage{mdwtab}
% \usepackage{eqparbox} %equations

% ---------------------------------
%Symbols
% ---------------------------------
\DeclareMathAlphabet{\mathcal}{OMS}{lmsy}{m}{n}
\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
\usepackage{textcomp} %for getting text tilde
%\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
%\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
%\usepackage{dsfont}

% ---------------------------------
%  Algorithms
% ---------------------------------
% http://tex.stackexchange.com/questions/229355/algorithm-algorithmic-algorithmicx-algorithm2e-algpseudocode-confused

\usepackage{algorithm} %float wrapper for algorithms. %dont use with algorithm2e
%should only use one of algorithmic or algorithmicx or algorithm2e
% \usepackage{algorithmic} %least preferred
% \usepackage[ruled,vlined,linesnumbered]{algorithm2e} 
\usepackage{algorithmicx, algpseudocode} %algpseudocode:layout for algorithmicx

% \algtext*{EndFunction}% Remove "end while" text
% \algtext*{EndWhile}% Remove "end while" text
% \algtext*{EndIf}% Remove "end if" text


% ---------------------------------
%Table Stuff
% ---------------------------------
\usepackage{array} %for table entries to be in center of cell
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs}

% ---------------------------------
%DOCUMENT WIDE
% ---------------------------------
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[english]{babel} %for hyphenation rules
\usepackage{units}
% \usepackage{siunitx}
\usepackage{bm}
\usepackage{times} % assumes new font selection scheme installed
\usepackage{xspace}
\usepackage{flushend}%balance columns on last page
% \usepackage[yyyymmdd,hhmmss]{datetime}
\usepackage{csquotes}
\usepackage{makeidx}
\usepackage{blindtext}
\let\labelindent\relax
\usepackage{enumitem}

% \usepackage{fixltx2e} %fix latex issue across versions not needed in new latex versions
\usepackage{soul} %text highlighting
\usepackage{subfiles} %individual file compilation--makes it quick 

\usepackage[protrusion=true,expansion=true]{microtype}
\setlength{\emergencystretch}{3em}

\usepackage[yyyymmdd]{datetime}
\renewcommand{\dateseparator}{-}
\date{\protect\formatdate{1}{1}{2001}}

% ---------------------------------
%Bibliography and cross-ref
% ---------------------------------
% The following lines are for IEEE style conflicts with natbibs
% \makeatletter
% \let\NAT@parse\undefined
% \makeatother
% \usepackage[numbers]{natbib}
% \usepackage{cite} %DONT USE NATBIB AND CITE TOGETHER

%hyperlinking
\usepackage{url}
\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother
\usepackage{color}
\usepackage[usenames,dvipsnames,table]{xcolor}
% \usepackage[pdfborder={0 0 0.5}]{hyperref}
% \usepackage{hyperref}
% \hypersetup{
%     colorlinks=true,
%     linkcolor=black,
%     citecolor=black,
%     filecolor=cyan,
%     urlcolor=black
% }

%=======U S E R  D E F I N E D  M A C R O S=======
% ---------------------------------
% User Comments
% ---------------------------------
\usepackage{marginnote}
% \newcommand{\bibhref}[2]{#2}
\newcommand{\todohl}[1]{{[\hl{#1?}]}}
% \usepackage[disable]{todonotes}
% \usepackage{todonotes}
\usepackage[colorinlistoftodos]{todonotes}
%takes in optional argument
% \newcommand{\tocite}[1]{%
% \textcolor{red}{[cite:\ifthenelse{\equal{#1}{}}{}{#1}?]}
% }

\newcommand{\animesh}[1]{\todo[inline,color=blue!20]{AG: #1}}
\newcommand{\ignore}[1]{}
\newcommand{\etal}{et al.~}

% ---------------------------------
% Label utils
% ---------------------------------

% Usage:
% \figlabel{myfigure} creates \label{fig:myfigure}
% \figref{myfigure} references it
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Fig.    \,\ref{fig:#1}}

% Usage:
% \seclabel{mysection} creates \label{sec:mysection}
% \secref{mysection} references it
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section\,\ref{sec:#1}}

\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter\,\ref{ch:#1}}

% Usage:
% \tablabel{mytable} creates \label{tab:mytable}
% \tabref{mytable} references it
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% space tweaks 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\abovecaptionskip}{0.5mm}
\setlength{\belowcaptionskip}{0mm} 
\setlength{\textfloatsep}{1.5mm}
\setlength{\dbltextfloatsep}{1.5mm}
%\renewcommand{\baselinestretch}{.9945}

\makeatletter
\newenvironment{mcases}[1][l]
 {\let\@ifnextchar\new@ifnextchar
  \left\lbrace
  \def\arraystretch{1.2}%
  \array{@{}l@{\quad}#1@{}}}
 {\endarray\right.}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% symbol definitions for equations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> 1-intro-v2.tex <==
\section{Introduction}
% P1: RL is hard, IL is a solution along with task structure from 

% IL can be batched or online. Batched has problems with covariate shift hence online can be preferred. 

% Online experts whether human or algorithmic help correct iterative policies in new state spaces while the agent itself is improving. 

% At the same time, task structure can be provided also through options. But it is arguably easier to create a set of heuristics -- potentially incapable of handling all possible cases, yet provide valuable information about the task structure to an RL agent. 

% This paper looks at the problem of ---- 


Recent research has successfully employed Reinforcement Learning (RL), Self-Supervised Learning (SSL), and Imitation Learning (IL) for short-horizon skill learning, such as pushing and grasping objects~\cite{yu2016more,levine2016learning,fang2018learning}. 
However, RL methods require reward specification, face the burden of efficient exploration in large state spaces, and need large amounts of interaction with the environment to collect sufficient data for policy learning.
SSL has been used successfully to collect and learn from large quantities of data in both simulated~\cite{mahler2017dex,kasper2012kit,goldfeder2009columbia} and physical settings~~\cite{levine2016learning,pinto2016supersizing,kalashnikov2018qt} for tasks such as grasping. However, the data has very low signal-to-noise ratio due to random exploration.
In contrast, IL uses expert demonstrations to reduce environment interaction during skill learning. Imitation Learning is commonly posed either as inverse reinforcement learning~\cite{abbeel2011inverse,ng2000algorithms} or behavioral cloning~\cite{argall2009survey,pomerleau1989alvinn}, both of which require demonstrations.
Prior works show that data-driven IL methods improve both the sample efficiency of policy learning~\cite{abbeel2010autonomous,vevcerik2017leveraging,krishnan2016swirl} and the performance of the trained policy~\cite{gupta2016learning,boularias2011relative,ho2016generative}.




We assume that the set of teachers can be imperfect in the following ways: (i) \textit{suboptimal} -- one or more teachers may recommend different actions than what the optimal policy would, (ii) \textit{partial} -- one or more teachers may recommend useful actions, but only in a part of the state space, (iii) \textit{insufficient} -- the agent cannot solve the task by only using actions suggested by the teachers, and (iv) \textit{contradictory} -- alternating actions from different teachers would impede task completion (see Figure 1).
In this work we present \textbf{Actor-Critic with Teachers (\methodname)}, an approach to learn a policy from advice from multiple teachers that can have any or none of these qualities.

We build on the framework of off-policy RL, where a separate \emph{behavioral policy} is used to gather experience for training the agent. The behavioral policy collects experience by selecting between the actions suggested by several teachers and the action from the training agent. Constructing a good behavioral policy is particularly challenging in this setting since the utility of the teachers varies in different state space regions while the utility of the agent varies over time.
% While this broad framework has been the basis of multiple past works\cite{ppr, opstl, wheels}, these prior works have either been focused on discrete grid worlds or on a setting with only a single teacher.
% A possible approach is to not model actions but to model the value of each teacher as well as the student~\cite{wheels}. 
% However, this approach has been only shown to converge for a single teacher, it does not take into account the changing performance of the learner policy, and it does not account for contradictory advice from teachers. 
% Differently, 
\methodname~ is a novel behavioral policy mechanism that for continuous control is robust to the four aforementioned teachers imperfections (i-iv) by measuring uncertainty over the actions effect based on a probabilistic posterior critic network~\cite{henderson2017bayesian} and using the uncertainty to choose between different action proposals. 
Using Bayesian probability-based selection accounts for the dynamically changing performance of the learning agent and enables temporally extended commitment to cope with contradictory advice. 

==> 8-discussion.tex <==
\section{Discussion}
negative results?

future work - parametrzied teachers? bcq + demonstrations as teacher?
